Population Protocols with Faulty Interactions: the Impact of a Leader

We consider the problem of simulating traditional population protocols under weaker models of communication, which include one-way interactions (as opposed to two-way interactions) and omission faults (i.e., failure by an agent to read its partner's state during an interaction), which in turn may be detectable or undetectable. We focus on the impact of a leader, and we give a complete characterization of the models in which the presence of a unique leader in the system allows the construction of simulators: when simulations are possible, we give explicit protocols; when they are not, we give proofs of impossibility. Specifically, if each agent has only a finite amount of memory, the simulation is possible only if there are no omission faults. If agents have an unbounded amount of memory, the simulation is possible as long as omissions are detectable. If an upper bound on the number of omissions involving the leader is known, the simulation is always possible, except in the one-way model in which one side is unable to detect the interaction.

==> impossibilitiesshort2.tex <==
% !TEX root = 1wayLeader.tex

\section{Simulation with a Leader  in Presence of Omissions: Impossibility \label{imp1}}


In this section we prove that
the presence of a leader, alone, might not be  sufficient to overcome dynamic omissions. Indeed, we  prove that
there are two-way protocols that cannot be simulated with omissive interactions even if a leader is present.
%
%Let us first  consider a property on the behavior of a generic simulator ${\cal S(\mathcal P)}$ of a two-way protocol ${\cal P}$ that will be useful in our proofs. Let us fix a sequence of interactions $I$ for a system of only two agents executing ${\cal S(\mathcal P)}$, and let us also fix an initial configuration $C_0$ (i.e., a pair of initial local states for the two agents). We define the {\em Transition Time} ({\sf TT}) of the triplet $({\cal S(\mathcal P)}, I, C_0)$ as the time at which both agents in the system have completed their first simulated transition as they execute protocol ${\cal S(\mathcal P)}$ from the initial configuration $C_0$ following the sequence of interactions $I$.
%
%We further define the {\em Fastest Transition Time} ({\sf FTT}) of the pair $({\cal S(\mathcal P)},C_0)$ as the smallest {\sf TT} of all the triplets of the form $({\cal S(\mathcal P)},I,C_0)$, where $I$ ranges over all possible sequences of interactions between two agents with no omissions.
%Intuitively, {\sf FTT} is the minimum number of (non-omissive) interactions needed by a specific simulator ${\cal S}$ to simulate a single two-way step of protocol ${\cal P}$ in a system of two agents. Thus it can be regarded as the \vir{maximum speed} of a simulator. It has been shown in~\cite{DiFIISV16} that such a metric is intrinsically related to the omission resilience of ${\cal S}$.


Next we consider the {\em Pairing Problem} (\textsf{Pair}), introduced in~\cite{DiFIISV16}:
a set of agents $A$ is given,  partitioned into  \emph{consumer} agents $A_c $,  starting in state   $c$, 
and \emph{producer} agents  $A_p$, starting in state $p$. 
We say that a protocol $\mathcal P$ solves the \emph{Pairing Problem} if it enforces the following properties:
\begin{enumerate}
\item[(i)] {\em Irrevocability:} $\mathcal P$ has a state $cs$ that only agents in state $c$ can reach; once an agent has state $cs$, its state cannot change any more;
\item[(ii)] {\em Safety:} At any time, the number of agents in  state $cs$ is at most $|A_p|$;
\item[(iii)] {\em Liveness:} In all globally fair executions of $\mathcal P$, eventually the number of agents in  state $cs$ is stably equal to $\min\{|A_c|,|A_p|\}$.
\end{enumerate}

This problem can be solved in the standard two-way model by the  simple protocol below:

\begin{framed}

\footnotesize
{\sf  Pairing  Protocol} $\mathcal{P}_{IP}$.
$Q_{\mathcal{P}_{IP}} = \{cs,c,p,\bot\}$.  The only non-trivial transition rules are $(c,p) \mapsto (cs,\bot)$ and $(p,c) \mapsto (\bot,cs)$.
\end{framed}

\noindent However, as we will show, this protocol  cannot be  simulated, in spite of the presence of a leader,  even in the simplest of the omissive models.



\subsection{Impossibility  with Bounded Memory \label{impossleader}}
We investigate what happens when we introduce a distinguished leader node, but  we restrict the memory of agents to be bounded by some function of $|A|$.
%Without a leader we have shown that, in some omissive models, the presence of a single omission is sufficient  to render the  two-way simulation impossible  (even in presence of infinite memory).
 %In this section we show that the situation is similar in presence of a leader, constraining the memory to be constant. The next Section will treat the case of leader and infinite memory.
% that the upper bound on the number of omissions is crucial to be able to simulate omissive models with a leader  because, if such an upper bound   is unknown, no  simulation is possible. 
We show our impossibility results directly for the {\sf T}$_3$ omissive model. The results clearly carries over to the one-way models.

 
%{\em We will show in Section \ref{} that the situation drastically changes when a leader is available  and an  upper bound  on the number of omissions is known, even with bounded   memory, in which case   it is possible to  tolerate any   constant number of omissions in all interaction models investigated. } This is contrast with the results wi




\begin{definition}{\bf ({Omission-Recurrent State})} Let $\{\ell,a\}$ be a system of two agents,  where $\ell$ is the leader, and let $C=(q_\ell,q_a)$ be a configuration. We say that $q_\ell$ is an \emph{omission-recurrent state} for protocol ${\cal P}$ and configuration $C$ if
there exists a finite non-empty sequence of interactions $I_{C}=(i_1,i_2,\ldots,i_t)$, with $i_1$ omissive on both sides, such that, if $I_C$ is executed according to the transition rules of ${\cal P}$ starting from configuration $C$, eventually the state of $a_\ell$ is again $q_\ell$. \label{def:rec}
\end{definition}
Note that, in the above definition, since $i_1$ is omissive on both sides, the system transitions into configuration $(o(q_\ell),h(q_a))$ or $(h(q_\ell),o(q_a))$ after executing $i_1$.

\begin{lemma} \label{lemma:rec}
Let $\mathcal{S}(\mathcal{P})$ be a simulator having $k$ states in total and working under the $\diamond${\bf NO} adversary ($k$ could be a function of the number of agents executing the protocol, but it is finite). Let a system of two agents $\{\ell,a\}$ be given, where $\ell$ is the leader. Let $C_0$ be an initial configuration for $\ell$ and $a$ and let $I=(i_1,i_2,\ldots)$ be an infinite sequence of interactions with no omissions between $\ell$ and $a$ such that, if $\mathcal{S}(\mathcal{P})$ is executed according to $I$ starting from $C_0$, then the execution is globally fair. Then there exists a finite sequence of interactions $I'=(i'_1,i'_2,\ldots\,i'_t)$ with the following properties.
\begin{enumerate}
\item[(1)] $I'$ is obtained by introducing at most $k$ omissive interactions into an initial finite sub-sequence of $I$. All the omissive interactions of $I'$ are omissive on both sides.
\item[(2)] If $\ell$ and $a$ execute $\mathcal{S}(\mathcal{P})$ according to $I'$ starting from $C_0$, they both change simulated state (according to $\delta_{\cal P}$).
\item[(3)] Suppose that $\ell$ and $a$ execute $\mathcal{S}(\mathcal{P})$ according to $I'$ starting from $C_0$, and let $C_j$ be the configuration of $\ell$ and $a$ immediately before executing interaction $i'_{j+1}$. Then, if $i'_{j+1}$ is not omissive, the local state of $\ell$ in $C_j$ is omission-recurrent for $\mathcal{S}(\mathcal{P})$ and $C_j$.
\end{enumerate}
\end{lemma}
\begin{proof}
First we will insert at most $k$ omissive interactions into $I$ (thus building an infinite sequence that satisfies property~(1)) in such a way as to satisfy property~(3). Then we will choose $t$ so as to satisfy property~(2).

We will construct $I'$ incrementally by an inductive procedure. Suppose we have constructed $I'$ up to $i'_j$, and let $C_{j}$ be the configuration of $\ell$ and $a$ after executing the first $j$ interactions of $I'$ starting from $C_0$ (the base case is with $j=0$). Suppose also that the partial sequence $(i'_1,\ldots,i'_j)$ has been obtained by adding some omissive interactions to some initial sub-sequence of $I$, say $(i_1,\ldots,i_{v(j)})$ (with $v(0)=0$, i.e., in the base case the sub-sequence is empty). Now, if the local state of $\ell$ in $C_j$ is omission-recurrent for $C_j$, we set $i'_{j+1}=i_{v(j)+1}$ and $v(j+1)=v(j)+1$. Otherwise, we let $i'_{j+1}$ be omissive on both sides, and we set $v(j+1)=v(j)$.

We claim that, if we continue this process indefinitely, we put at most $k$ omissive interactions in $I'$. Indeed, suppose that the local state of $\ell$ in $C_j$, say $q_\ell$, is not omission-recurrent for $C_j$, which causes the addition of the omissive interaction $i'_{j+1}$ to $I'$. By definition of omission-recurrent state, $\ell$ will never get state $q_\ell$ after executing $i'_{j+1}$. It follows that the same state $q_\ell$ will contribute to the addition of at most one omissive interaction to $I'$. Since the possible states for $\ell$ are $k$, there can be at most $k$ omissive interactions in $I'$.

We now have to decide when to stop the incremental construction of $I'$. Recall that the execution of $I$ starting from $C_0$ is globally fair, and observe that adding finitely many omissive interactions to it preserves its global fairness. So, by definition of simulator, the simulated states of $\ell$ and $a$ also change in a globally fair way as they execute $I'$. Therefore, at some point, they will conclude a simulated interaction, changing their local states according to $\delta_{\cal P}$. At this point we stop the construction of $I'$, obtaining a sequence of finite length $t$ that satisfies all three properties.
\end{proof}

\begin{theorem}\label{th:ledmemfinimp}
Given a leader and only a bounded amount of memory on each agent, it is impossible to simulate every  two-way protocol in the {\sf T$_3$} model (hence in all the \emph{omissive} models), even under the  $\diamond${\bf NO} adversary. 
 \end{theorem}
\begin{proof}
We will show that the Pairing Protocol ${\cal P}_{IP}$ cannot be simulated in {\sf T$_3$}. Suppose by contradiction that there is a simulator $\mathcal{S}(\mathcal{P}_{IP})$ for it, and let us consider a system of two agents $\ell$ and $a$, where $\ell$ is the leader. Let $C_0$ be an initial configuration in which $\ell$ has simulated state $p$ and $a$ has simulated state $c$ and let $I$ be an omission-less infinite sequence of interactions for the two agents whose execution starting from $C_0$ is globally fair. According to ${\cal P}_{IP}$, eventually $I$ will make both $\ell$ and $a$ change simulated state to $cs$ and $\bot$, respectively.

Let us apply Lemma~\ref{lemma:rec}, which yields a sequence of interactions $I'=(i'_1,\ldots,i'_t)$ of length $t$, some of which are omissive on both sides. The sequence $I'$ guarantees that both agents will change simulated state to $cs$ and $\bot$, as per property~(2). Let $C_j$ be the configuration of the two agents immediately after executing interaction $i'_j$. Now we construct a larger system of agents: $\{\ell, a, b_1, b_2, \ldots, b_m, c\}$, where $m=2^t$. Let $C'_0$ be the configuration of this system in which $\ell$ and $a$ have the same state as in $C_0$ and all other agents have the same state as $a$. We will show how to modify $I'$ by inserting some extra interactions in it, obtaining an extended sequence $I''$ that involves also the other members of the system (as opposed to only $\ell$ and $a$). We will then show that executing $I''$ makes the simulator behave in a way that is not compatible with the Pairing Problem.

We will construct $I''$ inductively by inserting a sequence of interactions before each interaction $i'_j\in I'$. Say we have already done so up to $i'_j$, with $0\leq j<t$ (the base case being with $j=0$). Executing $I''$ up to this point from configuration $C'_0$ makes the system reach configuration $C'_j$. Let $w(j)=m/2^j$ and suppose that agents $a$, $b_1$, $b_2$, \ldots, $b_{w(j)}$ have the same state in $C'_j$ (this is certainly true for $j=0$). Also suppose that, in $C'_{j}$, $\ell$ and $a$ have the same state as in $C_{j}$ (again, this is true for $j=0$). As we construct $I''$, we will also prove that these properties are preserved. Now consider the next interaction $i'_{j+1}$, which could be either non-omissive or omissive on both sides. Next we are going to explain what interactions we add to $I''$ between $i'_{j}$ and $i'_{j+1}$.

Suppose that $i'_{j+1}$ is omissive on both sides and let $\ell$ be the starter and $a$ the reactor. Then we introduce in $I''$ (right after $i'_{j}$) the sequence of interactions $(c,b_1)$, $(c,b_2)$, \ldots, $(c,b_{w(j)/2})$, omissive on both sides. Finally we introduce $i'_{j+1}$ into $I''$. If $a$ is the starter and $\ell$ the reactor, we insert the same interactions, but with starter and reactor exchanged. It is immediate to see that, after executing these interactions, $a$, $b_1$, $b_2$, \ldots, $b_{w(j+1)}$ have the same state again. Indeed, they have the same state in $C'_J$ and then they all execute one omissive interaction as starters or as reactors. Moreover, in $C'_{j+1}$, $\ell$ and $a$ have the same state as in $C_{j+1}$.

Suppose that $i'_{j+1}$ is not omissive and let $\ell$ be the starter and $a$ the reactor. By property~(3) of $I'$, the state $q_\ell$ of $\ell$ in $C_j$ (hence in $C'_j$) is omission-recurrent for $C_j$. Therefore there exists a sequence of interactions $R=(i^\ast_1,i^\ast_2,\ldots,i^\ast_z)$, with $i^\ast_1$ omissive on both sides, involving $\ell$ and $a$, such that 


Then we introduce in $I''$ (right after $i'_{j}$) the following interactions. For all $1\leq x\leq w(i)/2$, we 
\end{proof}

%
%We end this subsection by showing another relevant problem, and relative protocol, that cannot be simulated despite the presence of a leader.
%\begin{problem}[Irrevocable Naming Problem (\textsf{INP})]
%Given a set of agent $A$. $A$ contains an unique leader $a_s$ with initial state $id_{l_0}$, the other agents $a_j \in A \setminus \{a_s\}$ have state $\bot$.
%A protocol {\cal P} solves \textsf{INP} if it enforces the following properties:
%\begin{description}
%\item[Safety:]  An agent $a_j \in A \setminus \{a_s\}$  can only change its state $\bot$ to an irrevocable state, moreover if $a_j$ sets its state to $q_j$ there is no other agent $a_i \neq a_j$
%in the system with state $q_i=q_j$.
%\item[Liveness:] Eventually, each  $a_j \in A \setminus \{a_s\}$  has a state $q_j \neq \bot$.
%\end{description}
%\end{problem} 
%This problem could be relevant in many context: let us consider a mutual exclusion mechanism on distinguishable resources, once an agent has an unique state it can access exclusively the corresponding resource. It is easy to see that in the standard two-way with a leader and  ${\cal O}(\log n)$ bits of memory the problem {\sf INP} is solvable. Consider the following simple protocol.
%
%\begin{framed}
%{\sf Irrevocable Naming Protocol} $\mathcal{P}_{IN}$:
%$Q_{\mathcal{P}} = \{id_{l_0}, id_{l_1},\ldots,\bot,1,2,\ldots\}$.  \\The generic non-trivial transition rule is: $(id_{l_j},\bot) \mapsto (id_{l_{j+1}},j) $. \end{framed}
%
%It is easy to see that  $\mathcal{P}_{IN}$ solves {\sf INP}. However, it is also immediate that we can use Lemma \ref{lemma:leaderindstinguishability1} to show that $\mathcal{P}_{IN}$ cannot be simulated, the simulator ends up assigning the same state to $a_{r,1},a_{b,1}$.

\subsection{Impossibility  with Infinite Memory  \label{sec:impleaderinfmemory}}
For this case we can show that simulation is impossible in the omissive two-way model without detection, and thus in {\sf IO}. 

\begin{theorem} \label{th:infmemleader}
Given a leader and an infinite amount of memory on each agent, it is impossible to simulate every  two-way protocol in the {\sf T$_1$} model, even under the  $\diamond${\bf NO} adversary. 
 \end{theorem}
\begin{proof}
We show that there exists a protocol ${\cal P}$, an initial configuration $\pi_{\cal P}({C}_{0})$, a sequence of interactions $I$  inducing a {\sf GF} sequence of configurations, and an adversary ${\diamond}${\bf NO} where ${\cal S}$  fails to simulate ${\cal P}$. Let us consider the pairing protocol, a $C_{0}$ such that $\pi_{{\cal P}}(C_0)=(p,c)$ and a system composed by three agents $a_s,a_{r,1},a_{b,1}$  with states, respectively, $p,c,c$. Now let us consider a sequence $I$ with $TT^{*}=FTT^{*}$ for $({\cal S}, {\cal P}_{IP}, C_0)$. It is easy to see that we can keep $a_{r,1}$ and $a_{b,1}$ in the same state. Each time there is an interaction $(a_s,a_{r,1})$ we put a starter side omission $(a_s,a_{b,1})$, each time the interaction is  $(a_{r,1},a_{s})$ we put a reactor side omission $(a_{b,1},a_{s})$. So we can build a sequence $I'$ such that all agents $a_s,a_{r,1},a_{b,1}$ cannot distinguish it from a run of $I$ on $C_0$. Thus ${\cal S}$ set the simulated state of agents $a_{r,1},a_{b,1}$ to $cs$ violating the existence of a perfect matching on $E(\Gamma_I)$. \end{proof}


\begin{observation}
 It  is impossible to irrevocably simulate a {\sf TW} protocol in interaction model {\sf IO}
% $\delta(a_s,a_r):\{(f_s(a_s,a_r),f_r(a_s,a_r)),$\\$\{(a_s,f_r(a_s,a_r)), (f_s(a_s,a_r),a_r)\}\}$,
even under    $\diamond${\bf NO} adversary, presence of a leader,  and infinite memory.
\end{observation}


